METRO: Efficient Denoising Pretraining of Large Scale Autoencoding Language Models with Model Generated Signals

We present an efficient method of pretraining large-scale autoencoding language models using training signals generated by an auxiliary model. Originated in ELECTRA, this training strategy has demonstrated sample-efficiency to pretrain models at the scale of hundreds of millions of parameters. In this work, we conduct a comprehensive empirical study, and propose a recipe, namely "Model generated dEnoising TRaining Objective" (METRO), which incorporates some of the best modeling techniques developed recently to speed up, stabilize, and enhance pretrained language models without compromising model effectiveness. The resultant models, METRO-LM, consisting of up to 5.4 billion parameters, achieve new state-of-the-art on the GLUE, SuperGLUE, and SQuAD benchmarks. More importantly, METRO-LM are efficient in that they often outperform previous large models with significantly smaller model sizes and lower pretraining cost.

==> Figs/XXL.tex <==
\begin{figure}[t]
% \subfigcapmargin=10pt
% \vspace{-0.5cm}
\centering
\begin{subfigure}[t]{0.248\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figs/XXL_LR_replace_acc_plot.pdf}
	\caption{Replace Accuracy\label{fig:xxl_replace_acc}}
\end{subfigure}%
~
\begin{subfigure}[t]{0.248\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figs/XXL_LR_replace_rate_plot.pdf}
	\caption{Replace Rate \label{fig:xxl_replace_acc}}
\end{subfigure}
\caption{Pre-training curves with several hyper-parameters configurations for METRO-XXL: (a) represents the replace accuracy of the main model in pre-training, and (b) represents the replace rate of the auxiliary model in pre-training.
\vspace{-1em}
}\label{fig:XXL}
\end{figure}

==> Figs/init_res.tex <==
\begin{figure}[t]
% \subfigcapmargin=10pt
% \vspace{-0.5cm}
\centering
	\includegraphics[width=\columnwidth]{Figs/mnli_model.pdf}
	\caption{Scaling results of \model{} on MNLI-m test set w.r.t. different parameter counts. \cx{redraw one to differential with the one used in evaluation. Maybe we use time as x-axis, the left y as the model scale of notable large NLR+T5+METRO-XXL models and the right y as their performance on MNLI. It will show that ours are smaller but more powerful.}
	\label{fig:scale_res}}
\end{figure}

==> Sections/stabletune.tex <==
\section{Stable Fine-Tuning}
We enhance generalization and robustness of {\model} fine-tuning through posterior differential regularization (PDR) \cite{cheng2020pdr}, which is a fast and simplified version of virtual adversarial training \cite{miyato2018virtual, jiang2019smart, liu2020alum}. PDR directly promotes the model local smoothness, \eg stabilizing the model posterior distribution towards small input perturbations: 
\begin{eqnarray}
\min_\Theta L(f_\Theta(\xvec), \yvec) + \alpha R(f_\Theta(\xvec), f_\Theta(\hat{\xvec})),
\end{eqnarray}
where $\hat{\xvec} = \xvec + \epsilon$, $\epsilon\in\RR^n$ is a random vector bounded in a norm by $c$, $R$ is a regularization term penalizing the model instability, a small positive constant, and $\alpha$ is a hyperparameter for balancing the original task specific loss and the regularization term. In our experiments, we simply set $\alpha=1$.  

\input{Tabs/superglue}
\input{Tabs/glue}




==> Tabs/base_ablation.tex <==
% \cx{Payal TODO: Table of results of various combination of these techniques and baselines in GLUE Dev.}

\begin{table*}[t]
\centering
\caption{
Results on GLUE and SQuAD 2.0 development set in \textbf{Base Setting:}  BERT Base Size, Wikipedia + Book Corpus (16GB). All results are single-task, single-model fine-tuning. We use Spearman correlation for STS, Matthews correlation for CoLA, and accuracy for the rest on GLUE. {AVG$_\text{Large}$} is the average of the first four larger tasks on GLUE and AVG is the average of the eight tasks on GLUE. 
All baseline results unless marked by (Ours) are reported by previous research. All our methods use the standard 12 layer Transformer encoder with 768 hidden dimension, which include 85M parameters in the network. The rest parameters are from token embeddings. Together, the total parameters of methods with 32K vocabulary, 64K vocabulary, and 128K vocabulary are 110M, 134M, and 184M, respectively.  \cx{caption is too long... we need to move some to the main content. I also think we may directly discuard AVG and AVG-large scores for GLUE. We can move the metric name following Xiaodong's table style, which will make GLUE tasks table header more consistent with SQuAD, and also our caption shorter.}
%\cx{we can remove the total params and model params columns as they are redundant now.} 
%\cx{a tradition is to put table caption on top and figure caption below.}
}
\small 
\resizebox{\textwidth}{!}{
\begin{tabular}{ll*{9}{l}ll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{10}{c}{\textbf{GLUE Single Task}} & \multicolumn{2}{c}{\textbf{SQuAD 2.0}} \\ 
% \hline
% \cline{3-13}
\cmidrule(lr){2-11}\cmidrule(lr){12-13}
& \textbf{MNLI} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{RTE} & \textbf{MRPC} & \textbf{STS-B} & \textbf{AVG$_\text{Large}$} & \textbf{AVG} &
\textbf{EM} & \textbf{F1}\\
\midrule
\multicolumn{12}{l}{\textbf{Baselines}} \\ 
\midrule
ELECTRA ~\citep{clark2020electra}
&  86.0/85.3	& 90.0	&	91.9	&	93.4	&	64.3	&	70.8	&	84.9	&	89.1	& 91.9 &	83.7 & 80.5 & 83.3\\
 Backbone
& 89.0/88.5	&	92.0	&	93.5	&	94.2	&	70.1	&	85.7	&	91.0	&	91.5 &  92.1 & 88.3 &   83.8  &  86.7 \\
\midrule
\multicolumn{12}{l}{\textbf{Vocabulary Configurations}} \\ 
\midrule
Backbone + 32K uncased 
& 88.5/88.1	&	92.1	&	93.2	&	93.8	&	69.2	&	84.5	&	90.4	&	91.4 &  91.9 & 87.9  &  &  \\
Backbone + 64K cased 
& 88.4/88.3	&	91.9	&	93.4	&	92.1	&	69.7	&	82.7	&	90.9	& 91.4 &	91.1 &  87.5  &  &  \\
\midrule
\multicolumn{12}{l}{\textbf{Data Pre-processing}} \\ 
\midrule
Complete-Sent Mode  & 88.7/88.5	&	91.9	&	93.4	&	93.4	&	69.1	&	84.5	&	90.9	&	91.2	&	91.8    &   87.9	&	83.8	&	86.6\\
\midrule
\multicolumn{12}{l}{\textbf{Training Objectives}} \\ 
\midrule
Backbone + CLM  &  88.8/88.6	&	92.0	&	93.5	&	94.2	&	71.2	&	85.9	&	91.2	&	91.3	&	92.1 &  88.5	&	83.6   &	86.5	\\
Backbone + SCL & 88.9/88.4 & 92.1 & 93.6 &	94.3 &	71.9 &  86.3 &	91.9	&	91.6 & 92.1 & 	88.8 &	84.0 & 86.7 \\
Backbone + Replace MLM  & 88.7/88.6	&	92.0	&	93.2	&	94.6	&	69.7	&	84.1	&	90.7	&	91.4	&	92.1 &  88.1	&	83.6	&	86.5\\
Backbone + 1-choice cloze & 88.8/88.5	&	92.1	&	93.3	&	94.3	&	71.4	&	82.7 	&  90.0	&	91.1	&	92.1 &  87.9	&	83.3	&	86.2\\
\midrule
\multicolumn{12}{l}{\textbf{Architectural Variations}} \\ 
\midrule
Backbone + TUPE + RRP 
& 89.0/88.5	&	92.1	&	93.6	&	94.8	&	69.9	&	86.6	&	90.7	&	91.0 &  92.1 &  88.4  & 83.0 & 85.8  \\
Backbone + Pre-LayerNorm  \\
Backbone + RP Bins=64 & 89.0/88.6 &	92.1 &	93.7 &	93.7 &	71.0 &	85.2 &	90.9 &	91.4 &	92.1 &  88.4 &	83.7 &	86.4 \\
\midrule
\multicolumn{12}{l}{\textbf{Combinations: Each row represents an additional technique added to the previous row}} \\ 
\midrule
Backbone + CLM + Zero-dropout 
& 88.7/88.3	&	92.2	&	93.4	&	94.5	&	70.2	&	86.3	&	91.9	&	91.5 &  92.2 &  88.6  & 83.9 & 86.6  \\
 + RP Bins=64  & 88.9/88.5	&	92.2	&	93.5	&	94.7	&	72.1	&	84.5	&	91.2	&	91.3	&	92.3 &  88.5	&	83.7	&	86.6\\
+ Reset CLS  & 88.7/88.4	&	92.0	&	93.3	&	94.3	&	70.8	&	85.2	&	90.9	&	91.4	&	92.0 &  88.3	&	84.0 	&	86.8\\
+ No mask CLS & 88.8/88.5	&	92.0	&	93.6	&	94.5	&	71.6	&	85.2	&	90.0	&	91.5	&	92.2 &  88.4	&  84.2	&	87.1\\
 - CLM + CLM\_V2 
& 88.8/88.6	&	92.1	&	93.4	&	94.5	&	70.9	&	85.9	&	90.7	&	91.3 &  92.2 &  88.4  & 84.4 & 87.1  \\
+ Non-shared absolute position embedding
& 89.0/88.7	&	92.2	&	93.6	&	94.7	&	69.8	&	85.6	&	90.7	&	91.3 &  92.3 & 88.3  & 84.7 & 87.3  \\
 + Non-shared Bias in LM head b/w Gen and Disc 
& 89.0/88.8	&	92.2	&	93.9	&	94.6	&	71.9	&	86.3	&	90.7	&	91.5 &  92.4 &  88.7  & 84.3 & 87.2  \\
\midrule
\end{tabular}
}

% \vspace{-0.3cm}
\vspace{-0.5em}
\label{tab:base_ablation_res}
\end{table*}

==> arxiv/abs.tex <==

\begin{abstract}
In this paper, we present our efforts to more efficiently scale up language representation model (e.g., bi-directional encoders) using pretraining signals generated by auxiliary language models. 
This model-guided pretraining strategy, originated in ELECTRA, is confirmed to improve pretraining efficiency with more challenging training signals and an effective learning curriculum. 
We present the first handbook to scale up the ELECTRA-style models to billions of parameters, including thorough empirical studies on training and modeling techniques, observations on the pretraining stability issues at billions scale, and techniques to improve the parallel pretraining efficiency and stability.
Our final method, METRO, "Model Enhanced TRaining for DenOising Language Models", efficiently scaled language models up to 5.4 billion parameters, and, more importantly, achieved better performances on various language representation tasks, while using only about half of parameters and computation cost compared to previous state-of-the-art large scale models.
\end{abstract}

==> arxiv/eval.tex <==
\section{Evaluation Results.}
In this section, we first present evaluations on \model{}'s effectiveness in downstream applications and its scaling efficiency. Then we discuss its advantage and room for improvements.




\subsection{Results with Vanilla Fine-tuning}
% GLUE, SuperGLUE, SQUAD benchmarks
Table~\ref{tab:model_scale_res} lists the evaluation results with the vanilla fine-tuning setup. 
At all model sizes, METRO outperforms all the baselines on nearly all tasks and establishes the new state-of-at art for GLUE and SQuAD 2.0.  Note that \model{}$_\text{Large}$ model performs similarly and sometimes even better than previous XL and XXL models, while only using a fraction of their parameters and significantly reduced pretraining computing costs. This further demonstrate the benefits of the pretraining efficiency of the model-generated denoising objective.
At extra large sizes, \model{}$_\text{XL}$ and \model{}$_\text{XXL}$ also achieves best performances on nearly all tasks evaluated, showing the benefits of our method on both efficiency and capability.

% demonstrating the effectiveness of this ELECTRA-style framework and our selection of recent techniques.

Among the ELECTRA-style models, \model{} provides the best combination of effectiveness and efficiency. While using the same encoder configurations in \textit{base} and \textit{large}, \model{} yield improvements over the original ELECTRA model with large margins. It also outperforms COCO-LM on most tasks, while being a cheaper model without using sequence contrastive learning and with a simplified CLM formulation. It is the first one that effectively scales up this promising ELECTRA-style approach to billions of parameters and brings in the benefit of model-generated learning curriculum to LLMs.

In Table~\ref{tab:model_scale_res}, the results on smaller GLUE tasks from several large models are omitted, including \model{}$_\text{XXL}$. As models get bigger and bigger, we notice that they start to overfit the small tasks where training labels are limited. This leads to high variance in their testing results which is not informative. More sophisticated fine-tuning techniques are required to effective leverage LLMs in such tasks, as we discuss in next experiments.


%% details 
%% DON'T del them by Xiaodong Liu
%92.81500000000001 0.0013899999999998306 0.09999999999999432
%92.649 0.0009539999999999698 0.09000000000000341
%92.25899999999999 0.0036740000000000253 0.17499999999999716
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figs/pdr_mtdnn.png}
    
    \caption{Score distribution on MNLI-m/mm dev average of \model{}$_\text{XXL}$ with and without Posterior Differential Regularization (PDR) and Data Augmentation (DA).   \label{fig:ft_stragety} }
\end{figure}

%% TASK formulation



\subsection{Results with Stable Fine-Tuning}
\label{subsec:sft}

A typical way to improve GLUE and SuperGLUE leaderboard scores is the leverage multi-task training where LLMs are first fine-tuned on MNLI and then adapted to other tasks~\citep{liu-etal-2019-multi}. In this set of experiments, we first study the benefit of stable fine-tuning techniques on MNLI, the ``root'' task for GLUE and SuperGLUE and then show the empirical performance \model{} with stable fine-tuning.


Figure~\ref{fig:ft_stragety} plots the score distribution of \model{}$_\text{XXL}$ with different techniques after \cx{Xiaodong: XXX} random runs in the exact same environment. PDR improves both average accuracy and stability. Itself yields 0.4 accuracy boost on MNLI, which is even more than beefing up \model{} from \textit{large} to \textit{XL}, or from \textit{XL} to \textit{XXL}. 

In this section, we study importance of stable fine-tune, in other words PDR \cite{cheng2020pdr},  on {\model-XXL} which includes 5.4B parameters and obtains SoTA performance on MNLI. We further study whether multi-task learning (MTL) which has a regularization effect via alleviating overfitting to a specific task \cite{caruana1997multitask,liu2019mt-dnn} helps PDR as well. We present our results in Figure~\ref{fig:ft_stragety}. On the MNLI development set including both matched and mismatched subsets, PDR (denoted as XXL+PDR) obtains average 0.4\% improvement over the standard fine-tuning approach (XXL) and retains smaller variance. By incorporating ANLI and SNLI tasks as MTL training (denoted as XXL+PDR+DA), it further boosts performance around 0.2\% over XXL+PDR. 



\subsection{Scaling Efficiency}
Figure \ref{fig:mnli_squad_results} summarizes the results for METRO models at various sizes along with baselines as well as at several pre-training stages. \ref{fig:mnli_model} demonstrates that METRO outperforms all baselines for all model sizes. Also it is more efficient, METRO-base is comparable to RoBERTa-large. Similarly, \ref{fig:squad_model} demonstrates that METRO outperforms all baselines for all model sizes except DeBERTa at 1.5B. We found that Disentangled attention greatly helps in improving SQuAD.

Figure \ref{fig:mnli_time} and \ref{fig:squad_time} show that METRO performance improves with more pre-training. The results for METRO-XXL for less than 90\% training are using a limited hyper-parameter search space due to costly fine-tuning. \cx{Discuss more insight here?}
\cx{I am also thinking we can move Figure 4 (a) and (v) to Intro to show our empirical gain in the beginning to deliver a strong first impression. We shall also add stable tune results in Figure 4 as one final data point.}

\input{Figs/results}
\cx{figure curves of \begin{enumerate}
    \item model size versus performance
    \item pretraining steps versus performance various pretraining sizes
    \item pretraining hours versus performance
\end{enumerate} 
}



\subsection{Discussions}
\cx{Discuss the challenges we have faced in this journey, list things that we think need more research to figure out in future research?}

\pb{the impact of scaling model up reduces - going from XL to XXL gives only 0.1 gain in average of large tasks}
\pb {adaptive LR - future work}






==> arxiv/exp.tex <==
\section{Experimental Methodologies}
% \cx{Add general idea of what this section is about here. Also discuss why we start with presenting the experimental methodologies first (because we need to first find the best base model setup to scale up.}
In this section, we describe experiment setup including the model configurations, datasets and evaluation methods used. We present these details here and refer them in next section while discussing ablations for the best base model setup.


\textbf{Pretraining Setup.} 
We evaluate our model with \textit{base} configuration which is similar to BERT$_\text{base}$ setting~\citep{devlin2019bert}. We train this model for 256M samples with batch size 2048 for 125K steps with 512 length sequences. We evaluate the impact of several vocabulary sizes as well as vocabulary case in our experiments. We train \textit{base++}, \textit{large++}, \textit{XL++} and \textit{XXL++} for 4B samples similar to RoBERTa. We use batch size of 2048 for 2M steps with 512 length sequences. We use linear warm-up followed by linear decay for all training experiments where the peak LR is decreased with larger models to stabilize training.


\textbf{Pretraining Corpus.} 
For \textit{base} models, the training corpus consists 16 GB text from Wikipedia and BookCorpus~\citep{zhu2015aligning}. For \textit{base++}, \textit{large++}, \textit{XL++} and \textit{XXL++} models, the training corpus consists of 160 GB text from Wikipedia, BookCorpus~\citep{zhu2015aligning}, STORIES~\citep{trinh2018simple}, CC-News~\citep{liu2019roberta} and OpenWebText~\citep{Gokaslan2019OpenWeb}.

\textbf{Downstream Evaluation.} 
We evaluate all the models on sequence level tasks such as GLUE~\citep{wang2018glue} and SuperGLUE~\citep{wang2019superglue} as well as SQuAD~\citep{rajpurkar2016squad} reading comprehension task. For vanilla fine-tuning, we fine-tune the model separately for each task and report the median of 5 random seeds. For leader board submissions, we apply advanced fine-tuning, ensemble and regularization techniques discussed later in the paper.


\textbf{Implementation Details.} Our work builds upon the open-source implementation of
MC-BERT~\cite{xu2020mc} and fairseq~\cite{ott2019fairseq}. More details about our implementation are present in Appendix.




==> arxiv/intro.tex <==
\section{Introduction}

% \cx{Intro outline:
% \begin{enumerate}
%     \item the state of large language models (LLMs). auto-regressive and representation models.
%     \item the concern of computing cost and potential diminishing return under the scaling law.
%     \item challenge of the limited scaling factor: One challenge is the static denoising training signal that limits the scaling factor the other is on training stability. reduced LR etc.
%     \item our goal is to leverage the machine generated training signal to more efficiently pretrain LLMs. Our work is
%     \item we first provide a thorough emprical studies of modeling techniques, then leverage DeepSpeed and FastPT to further improve efficiency
%     \item We also show observations of training instability during the LLM training process, one of the first empirical observations on the training issues, and also the practical techniques to mitigate some.
%     \item stable fine-tuning techniques at the scale of billions parameters. overall achieves SOTA on various setups.
% \end{enumerate}
% }

Scaling up language models---pretraining Transformers with a large amount of parameters on language modeling tasks---is a new frontier for language technologies. With heavy investment in the community, the parameters large scale language models (LLMs) have increased from hundreds of millions to trillions within five years~\citep{raffel2019t5, brown2020language, MT-NLG}.
Increasing the capacity of pretrained models does yield empirical advantages~\citep{wang2018glue, liu2019roberta, devlin2019bert, raffel2019t5},  and when reaching a certain scale, e.g., billions of parameters, LLMs start to show  few-shot and zero-shot abilities in certain language tasks~\citep{brown2020language, sanh2021multitask}, making them an interesting potential path to acquire more general intelligence.

On the other hand, multiple observations also pointed to the logarithmic scaling law of LLMs~\cite{kaplan2020scaling}: a linear empirical improvement in downstream tasks often require exponentially more parameters and computing resources. This is less ideal as it implies the diminishing return on the investment in further scaling LLMs and the capped ceiling when we hit the bound of computing resource. Recent research pointed out two challenges contributed to this unideal scaling factor: \textit{Static Training Signal}, the same  signals are used pretrain LLMs from beginning to the end, thus when models get stronger latter in the pretraining process~\citep{meng2021coco}, the signals, often randomly constructed, may no longer be strong enough to push the model; \textit{Optimization Stability}, training LLMs yield various stability issues and often has to reside to significantly smaller learning rates to avoid divergence, a less efficient usage of computing resources~\cite{xiong2020layer, liu2020understanding, shleifer2021normformer}.


In this paper, we seek to more efficiently scale up pretrained LLMs, specifically, non-autoregressive Transformers for language representation tasks, using dynamic training signals generated by an auxiliary model. The idea of more efficient pretraining with model-generated signals is originated in ELECTRA, where \citet{clark2020electra} leverages an auxiliary Transformer, pretrained side-by-side with the main models, to produce denoising signals that start easy and become hard as pretraining goes on. 
This natural learning curriculum addresses the \textit{Static Training Signal} challenge and is later revealed as the main contributor to ELECTRA-style models' pretraining efficiency~\citep{meng2021coco}. In this work, we provide a thorough empirical study of various techniques developed in this ELECTRA-style models and choose the best combination of techniques based on their effectiveness, efficiency, and simplicity, to form our method, "Model Enhanced TRaining for DenOising Language Models", \model{}. 

Then we develop the first receipts to scale up \model{}, the largest ELECTRA-style LLMs to date, including the best configurations and also how to leverage customized CUDA implementations and ZERO optimizer for more stable and efficient parallel training~\citep{rajbhandari2020zero}.
We also share our observations on the \textit{Optimization Stability} issues at the billions scale, and techniques to mitigate them. With these techniques together, we effectively scaled \model{} to five billions of parameters and achieved state-of-the-art empirical results in a large set of language representation tasks in GLUE, SuperGLUE, and SQuAD. More importantly, \model{} obtained better scaling factors, often achieving the same performance with previous LLMs using half of their parameters or pretraining computing costs. 

At the scale of billions of parameters, fine-tuning LLMs also suffers from instability issues. The model becomes too powerful and starts to overfit the fine-tuning task, especially if the amount of fine-tuning labels is limited. To improve the downstream performance of \model{}, we provide a receipt that improves its fine-tuning using multi-task learning and posterior differential regularization. These techniques further elevated \model{}'s effectiveness, help it achieve the state-of-the-art on both GLUE and SuperGLUE leaderboard. 
% Notably, \model{} is the first to outperform human performance on MNLI and RTE, which marks an empirical checkpoint that LLMs have achieved human performances on all GLUE tasks.

After discussing related work in the next section, we present the experiment setups for our studies in Section 3, and then details of \model{} in Section 4. In Section 5, we discusses our process of scaling up \model{} to billions of parameters, followed by the stable fine-tuning techniques in Section 6. We show the empirical results and analyses in Section 7 and conclude in Section 8.







==> arxiv/main_results.tex <==
\begin{table*}[t]
\centering
\caption{
Results on GLUE and SQuAD 2.0 development set in. All results are single-task, single-model fine-tuning. We use Spearman correlation for STS, Matthews correlation for CoLA, and accuracy for the rest on GLUE. {AVG$_\text{Large}$} is the average of the first four larger tasks on GLUE and AVG is the average of the eight tasks on GLUE.  \cx{we can update the style of this table following table 1 updates. I am also thinking move Xiaodong's METRO-Dev in Table 4 as METROC-XXL (Stable Tune).}
}
\small 
\resizebox{\textwidth}{!}{
\begin{tabular}{lll*{10}{l}ll}
\toprule
{\textbf{Model: Bigger Training Data,}} & {\textbf{Total}} & \multicolumn{10}{c}{\textbf{GLUE Single Task}} & \multicolumn{2}{c}{\textbf{SQuAD 2.0}} \\ 
% \hline
% \cline{3-13}
\cmidrule(lr){3-12}\cmidrule(lr){13-14}
{\textbf{and More Training Steps}} & {\textbf{Params}} & \textbf{MNLI-(m/mm)} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{RTE} & \textbf{MRPC} & \textbf{STS-B} & \textbf{AVG$_\text{Large}$} & \textbf{AVG} &
\textbf{EM} & \textbf{F1}\\
\midrule
\textbf{Base++} \\
\midrule
XLNet~\citep{yang2019xlnet} & 110M
& 86.8/- & 91.4 & 91.7 & 94.7 & 60.2 & 74.0 & 88.2 & 89.5 & 91.2 & 84.6 & 80.2 &--\\
RoBERTa~\citep{liu2019roberta} & 125M
& 87.6/- & 91.9 & 92.8 & 94.8 & 63.6 &  78.7 & 90.2 &  91.2 & 91.8 & 86.4 & 80.5 & 83.7\\
UniLM V2~\citep{unilmv2} & 110M
& 88.5/- & 91.7 & 93.5 & 95.1 & 65.2 & 81.3 & 91.8  & 91.0 & 92.2 & 87.1 & 83.3 & 86.1\\
% ELECTRA~\citep{clark2020electra} \\
DeBERTa~\citep{he2020deberta} & 134M
&  88.8/88.5 &--&--&--&--&--&--&--&--&--& 83.1 & 86.2 \\
% \hline
COCO-LM~\cite{meng2021coco}  & 134M 
& 90.2/90.0
 &	92.2 &	94.2 & 94.6 & 67.3 &	87.4 & 91.2 & 91.8 & 92.8  & 88.6 & 85.4 & 88.1 \\
\model{} & 184M & 90.3/90.2 & 92.4  &   94.4    &	95.87   &	71.8   &	88.1   &	91.4   &	92.0   &	93.2 & 89.5   &   85.9	&   88.5\\
\midrule
\textbf{Large++} \\
\midrule 
XLNet~\cite{yang2019xlnet} & 360M
& 90.8/90.8 &	92.3 &	94.9 &	97.0 &	69.0 & 85.9 &	90.8 &	92.5 &  93.8	& 89.2 & 87.9 & 90.6 \\
RoBERTa~\cite{liu2019roberta} & 356M
& 90.2/90.2 &	92.2 &	94.7 &	96.4 &	68.0 &	86.6 &	90.9 &	92.4 &  93.4 &	88.9 & 86.5 & 89.4 \\
ELECTRA~\cite{clark2020electra} & 335M
& 90.9/- & 92.4 & 95.0 & 96.9 & 69.1 & 88.0 & 90.8 & 92.6 & 93.8 & 89.4 & 88.0 & 90.6 \\
DeBERTa~\cite{he2020deberta} & 384M
& 91.1/91.1 & 92.3 & 95.3 & 96.8 & 70.5 & -- &-- &-- & 93.9 & -- & 88.0 & 90.7 \\ 
COCO-LM~\cite{meng2021coco} & 367M
& 91.4/91.6 & 92.8 & 95.7 & 96.9 & 73.9 & 91.0 & 92.2 & 92.7 & 94.2 & 90.8 & 88.2 & 91.0 \\ 
\model{}  & 434M & 91.7/91.7  &	92.9  &	95.8 &	96.3 &	75.2    &	93.1    &	92.2 &	92.8 &	94.2 & 91.3 &	   88.5 &	91.1 \\
\midrule
\textbf{XL++ and XXL++} \\
\midrule
Megatron$_\text{1.3B}$~\cite{shoeybi2019megatron} & 1.3B
 & 90.9/91.0 & 92.6 &--&--&--&--&--&--&--&--& 87.1 & 90.2 \\
Megatron$_\text{3.9B}$~\cite{shoeybi2019megatron} & 3.9B
& 91.4/91.4 & 92.7 &--&--&--&--&--&--&--&--& 88.5 & 91.2
\\
\model{}-XL & 1.6B &  92.2/92.0 &	93.2 &	96.3    &	97.3 &	76.0     &	93.5     &	91.7 &	93.0    &	94.7	& 91.6   &		89.4    &	92.1\\ 
\model{}-XXL  & 5.4B & 92.3/92.4 &	93.1  &  96.5   &	97.3    &	-    &	-    &	- & -	& 	94.8 & - & 89.7	& 92.4\\
\midrule
\end{tabular}
}

% \vspace{-0.3cm}
\vspace{-0.5em}
\label{tab:model_scale_res}
\end{table*}

==> arxiv/model.tex <==
\section{Pretraining Models and Techniques}

\cx{need a model figure that describes the final architecture of METRO.}


In this section, we first describe the preliminaries for METRO pre-training framework. We first start with ELECTRA~\citep{clark2020electra} which is the one of the first techniques to employ machine augmented signals to pre-train natural language representation models from unsupervised textual data. We then briefly discuss recent works that have extended this framework and demonstrated its advantages for several downstream applications. Motivated by this research, we present a thorough study of several pre-training techniques in this framework along with evaluation rooted in systematic ablation analysis to build an effective pre-training recipe.

\subsection{Preliminaries}
\cx{We need to elevate the generality of this preliminary description. While we be very careful to assign credit to ELECTRA being the inventor of this METRO framework, later research also made significant contribution to it. Our position now is to treat this general pretraining methodology as METRO, describe its general and core setup: using auxiliary model to generate denoising signals, and trains the main model to recover the original. Then we describe the main benefit of this setup in the curriculum learning. After that we conclude by going through different instantiation of this setup, including ELECTRA, MC-BERT, COCO-LM, and AMOS.}

In this section, we first present the pre-training framework for a family of models trained using machine generated and continuously evolving signals. The paradigm consists of the main model which is being pre-trained and planned to use for downstream tasks and one or more auxiliary models that create denoising training signals for the main model. Given an input $X$, the auxiliary model $M_{aux}$ is trained using a loss function $L_{aux}$. This auxiliary model transforms the input $X$ to $X^'$. This is then fed to the main model $M_{main}$ which is trained to denoise this input using $L_{main}$. Both models are trained together end-to-end.
\begin{align*}
   X \xrightarrow{\text{$M_{aux}$}} \bs{X'} \xrightarrow{\text{$M_{main}$}} Denoise(X')\\
  \mathcal{L}_{\text{model}} = \mathcal{L}_{\text{aux}} + \mathcal{L}_{\text{main}} \label{eq:dual_model}
\end{align*}

In previous works such as BERT, RoBERTa, AlBERT, etc. trained using Masked Language Modeling (MLM), a random set of tokens are masked irrespective of whether the model has already learned those training signals or not. Also, the signals are static, that is, the complexity of the task doesn't evolve over time. The advantage of employing an auxiliary model $M_{aux}$ is that training signals are not random and static. Unlike single model frameworks, in the auxiliary-main model framework, $M_{aux}$ is continuously training and producing more challenging signals for the main model $M_{main}$ and this curriculum between the two models makes the training more efficient. Several models in recent research follow this pre-training paradigm. We first describe ELECTRA ~\citep{clark2020electra} as it is one of the first models proposed in this framework and then present several works that build on top of this framework. 

ELECTRA employs BERT-style encoder as the auxiliary model $M_{aux}$ which is trained using Masked Language Modeling (MLM) task~\citep{devlin2019bert}. Given an input sequence $X=\{x_1, x_2, ...,x_i, ..., x_n\}$, 15\% of tokens are randomly masked with $\texttt{[MASK]}$ token to create a masked sequence $X_{mask}=\{x_1, x_2, ...,\texttt{[MASK]}_i, ..., x_n\}$ and the generator is trained to predict the correct tokens at masked positions $\mathcal{M}$:
\begin{align}
p_{\text{MLM}} (x_t | \bs{h}_i) = \frac{\exp(\bs{x}_t^\top \bs{h}_i)}{\sum_{t'=1}^{|V|} \exp(\bs{x}_{t'}^\top \bs{h}_i)}
\\
\quad
\mathcal{L}_{\text{aux}} = \mathbb{E} \left( - \sum_{i\in \mathcal{M}} \log  p_{\text{MLM}} \left( x_i^\text{orig} \big| \bs{h}_i \right) \right) \label{eq:gen}
\end{align}
where $\{\bs{h}_i\}_{i=1}^n$ are the contextualized representations generated by the Transformer (after the projection head) and $\{\bs{x}_t\}_{t=1}^{|V|}$ are the token embeddings.

The main model $M_{main}$ is constructed by sampling from the output probability distribution of the auxiliary model: 
\begin{align}
  x_i^\bs{'} \sim p_{\text{MLM}} \left(x | \bs{h}_i \right),\, \text{if $i \in \mathcal{M}$ };
  \quad
  x_i^\bs{'} = x_i,\, \text{else.} \label{eq:disc}
\end{align}
The main model $M_{main}$ is a transformer model trained using Replaced Token Detection (RTD) task where the output encodings are fed to a a sigmoid linear layer which outputs a binary probability to predict if the input token is original or replaced, and the main transformer is trained with binary cross entropy loss:
\begin{align}
\mathcal{L}_{\text{main}} = - \sum_{i=1}^n \log  p_{\text{main}} (x_i | x_i^{main}) \label{eq:disc_loss}
\end{align}
The pre-training loss is the weighted sum of auxiliary and main model loss:
\begin{align}
\mathcal{L} = \mathcal{L}_{\text{aux}} + \lambda \mathcal{L}_{\text{main}}  \label{eq:total_loss}
\end{align}
Both auxiliary and main models are trained together. As training progresses, the auxiliary model learns to predict more correct or semantically similar tokens making it more challenging to detect if the token is replaced for the main encoder. Recent research has demonstrated that curriculum learning is the key to this auxiliary-main model framework where the joint training provides the advantage of better training signals throughout the training compared to random masking of tokens thus making this framework efficient and effective. 

Several recent works have extended ELECTRA and more generally the auxiliary-main model framework using improvements in architecture, objectives, training signals as well as transfer it to different domains. \citep{meng2021coco} underlines the importance of jointly training the auxiliary and main model by demonstrating that modifying the training in two stages where auxiliary model is trained to convergence first followed by training the main model in second stage which yields a far inferior natural language representation model. cite(xlm) demonstrates the effectiveness of this framework in cross lingual model pre-training with much lower computational cost. cite(amos) proposed an approach to further improve this curriculum by training multiple auxiliary models simultaneously to provide better training signals to the main model. 

% Similarly, BART (ref) presents another example of training t

\subsection{Searching for Best \textit{Base} Model}

% \cx{As hinted in the title change, our goal in this subsection is to find the best combination in the base set, to have the backbone to scale up. We can start with this statement, plus the key principles we use to find the best techniques to include in the main model: 1) simplicity/efficiency 2) stability 3) effectiveness. Then we describe the baseline model we start with. After that, we can lead the general classes of techniques we explore, and then the details of each class. (We may also draw a figure of the techniques in a tree.}

In this section, we first describe our backbone implementation motivated by recent research in auxiliary-main model setup. We then discuss and evaluate several techniques on top of this backbone to create the best base model pre-training setup. The goal of this exploration is to find the best combination of techniques to create a pre-training recipe that is efficient, stable and effective. 

\textbf{Backbone Implementation:} 
% \cx{move this to the beginning of next subsection. Framing it as our baseline/backbone setup where we start the exploration from. It will be nice if we already have the description of METRO-style models, e.g., COCO-LM, in the end of previous part (instantiation), then here we can be concise for them.}
Similar to ELECTRA, we use a smaller auxiliary Transformer than the main model. Following COCO-LM~\citep{meng2021coco}, we replace the shallow and wide auxiliary model with a deeper and narrow architecture. Following T5~\citep{raffel2019t5}, we enable relative position embeddings for both the auxiliary and main model where we use 32 relative position bins. Following \citep{he2020deberta}, we use a cased sentencepiece BPE vocabulary of 128K tokens. The motivation of using a larger vocabulary it to leverage this additional capacity for scaling up. To create training samples, we respect the document boundaries such that every training sample consists of text only from one document. We don't concatenate text from different documents to create a training example. We present ablations on alternate data-processing, and vocabulary size and casing later in the paper.

\subsubsection{Baseline and Explored Techniques}
Since the advent of pre-training natural language representation models using transformers, several techniques have been proposed to leverage them effectively in this setup. These cover several domains such as the way pre-training data is created, pre-processed and presented to the model, what types of architectures enable training efficiently (deberta, ~\citep{ke2020tupe}) and scaling up to larger model size ~\citep{shoeybi2019megatron} as well as which training process provide more meaningful signals to the model such as span masking task ~\citep{joshi2019spanbert}, corrective language modeling task ~\citep{meng2021coco}, contrastive learning techniques (xlme). We experiment along all these axes in the auxiliary-main model setup where we apply these techniques in the pre-training stage followed by fine-tuning on downstream tasks for evaluation.\\


\textbf{Data related techniques:} Pre-training data quality, data processing to create training samples from text as well as the tokenization can be a determining factor in model performance. Here, we experiment with the following data related techniques:
% \cx{a general intro sentence here. Do not miss this opportunity to organize readers.}

\textit{Data Pre-processing}: We created the training samples by respecting sentence boundaries but not document boundaries, as a result of which it is possible that a training sample can consist of sentences from different documents at document boundaries. The training samples shorter than maximum sequence length were padded. 
% \cx{balance the detail/description level. I think we can be more concise.}

\textit{Vocabulary}: We evaluated the impact of different vocabulary configurations. First, we evaluate the impact of reducing vocabulary size from 128K BPE tokens to 64K BPE tokens. Second, we evaluate the impact of casing with 32K uncased BPE tokens.


\textbf{Architectural Variations:}Model architecture can play a key role in performance ~\citep{lan2019albert} as well as training stability ~\citep{shoeybi2019megatron}. We experimented with the following architectures:
% } \cx{say 1-2 sentences about your insights on the role of architecture in LLMs, your reflection of fields currently, and you intuition of picking the following techniques to experiment with.} 

 \textit{TUPE} We evaluated TUPE~\citep{ke2020tupe} which included the following changes: modified positional encoding method where the word and position correlations are decoupled with different weights and then summed together, and modified attention module where position correlations for [CLS] token are reset to learnable parameters. 
 
 \textit{Pre-LayerNorm} We evaluated the impact of changing the position of LayerNorm to before the self-attention and FFN in the transformer architecture similar to ~\citep{xiong2020layer}.

\textit{Relative Position Bins} We evaluated the impact of modifying the number of relative position bins to 64.


\textbf{Training Objectives:} The loss functions are crucial to determining the training signals are used to update model parameters. Recent studies have shown the importance of improving objectives, examples include: span masking provides better signal than random masking ~\citep{joshi2019spanbert}, sentence ordering provides a better signal than NSP task ~\citep{lan2019albert}. Here, motivated by recent research, we experiment with 4 different objectives:
% \cx{same intro sentence needed as previous groups}

\textit{Corrective Language Modeling (CLM)}: A language model head is added to the main model which uses the hidden representations $\bs{h_i}$ of a token to output a language modeling probability and is trained to predict the correct token. We enable CLM task only for masked tokens instead of all tokens and omit the copy mechanism to simplify the training process, unlike the original paper ~\citep{meng2021coco}:
\begin{align*}
  p_\text{CLM}(x_i | \bs{h}_i) &= \frac{\exp(\bs{x}_i^\top \bs{h}_i)}{\sum_{x_t \in V}\exp(\bs{x}_t^\top \bs{h}_i)}.
\end{align*}

\textit{Sequence Contrastive Learning (SCL)}: Following ~\citep{meng2021coco}, we create augmented data $X_{crop}$ by cropping the original sequence $X$ and apply a contrastive learning objective upon the sequence embeddings to learn more robust representations. The positive pairs are created from the same input sequences $\{X^{m}: (X^{m}_{mask}, X^{m}_{crop})\}$ and the negative pairs are all remaining sequence pairs in the batch: $X^{-}:\{(X^{m}_{mask}, X^{n}_{crop}), (X^{n}_{mask}, X^{m}_{crop})\}, m \neq n$.

\begin{align}
    \mathcal{L}_\text{\scl} &= -\mathbb{E}\left( \log \frac{\exp(\text{cos}(\bs{s}, \bs{s}^+)/\tau)}{\exp(\text{cos}(\bs{s}, \bs{s}^+)/\tau) + \sum_{X^-\in B^- } \exp(\text{cos}(\bs{s}, \bs{s}^-)/\tau)} \right),\nonumber \label{eq:scl}
\end{align}

where $\bs{s}, \bs{s^+}, \bs{s^-}$ are the representations of $X, X^+, X^-$, respectively, from the main Transformer (\textit{i.e.}, $\bs{h}_{\texttt{[CLS]}}$). 

\textit{Replace MLM}: The replaced token detection (RTD) task is removed and instead a LM head is added to the discriminator to predict the corrupted token. 
\textit{1-choice cloze}:
\cx{this part is not finished, broken eqn and unfinished paragraph.}



\subsection{Evaluation Results on \textit{Base}}



In this section, we discuss the evaluations of techniques presented above. The goal of this analysis is to understand their impact in auxiliary-main model setup and to study these ablations to create the best base model setup. We apply these techniques in model pretraining in $base$ setup and fine-tune the pre-trained model on downstream tasks $GLUE$ and $SQuAD$. For the purpose of these evaluations, we mostly focus on large tasks in $GLUE$, that is $MNLI$, $QNLI$, $QQP$ and $SST-2$ as well as $SQuAD$. Small tasks in $GLUE$ benchmark have shown to have high variance in results and thus might accurately represent the effect of a technique. \cx{move the description part in Table 1 caption here.}

\textit{Data related techniques}: We observed that reducing the vocabulary size and making it uncased leads to inferior performance. We observe that modifying the data pre-processing to complete sentence mode results in inferior performance compared to complete doc mode on GLUE. This is expected because training samples spanning documents can be confusing for the model for language modeling tasks.\\

\textit{Architectural Variations:} We observed that TUPE hurts SQuAD performance by a significant margin and PreLayerNorm provides inferior results despite of more stability in pretraining. \\

\textit{Training Objectives:} We observed that adding CLM objective provides a small boost in GLUE average results. Adding SCL objective provides gains, it is 44\% more computationally expensive than backbone which can be restrictive in scaling up. Adding Replace MLM hurts GLUE average, and 1-choice cloze task hurts both GLUE and SQuAD results.\\




\textit{Combinations.} After evaluating all the techniques individually, we worked on evaluating the impact of combining them. This design is motivated by performance on large GLUE tasks as well as SQuAD as we have observed larger variance in small task performance in GLUE. We started with CLM as it provides best gains in GLUE without any additional cost. We modified the generator training to use zero-dropout instead of eval mode to save on the cost of running generator twice and we observed that this doesn't affect performance. We modified relative position bins to 64 as it provides some gain in MNLI as well as average of large tasks. We then added reset the positional correlations related to [CLS] similar to ~\citep{ke2020tupe} which provides a boost in SQuAD performance. We observed that identifying if [CLS] is replaced or not can be an easy task for the discriminator which doesn't provide any training signal, so we removed masking [CLS] token and this further provides a boost in SQuAD. We noticed that training model with CLM can lead to instability. So we modified the CLM implementation, referred to as CLM\_V2 and simplified it to remove FC layers unlike the original paper implementation ~\citep{meng2021coco}. We observed that these modification lead to increased stability with comparable or better metrics. We then modified the architecture to not share absolute position embeddings and LM head bias between the auxiliary and main model. 


\textbf{Final \model{} Model.} \cx{recap the final setup of our model here.}
Our final model We adopt this combination and then scale it to larger model, data and longer training setups.




\input{Tabs/base_ablation}

==> arxiv/scale.tex <==
\section{Scaling Up to Billions of Parameters}

\input{Tabs/model_configs}

After finding a reliable configuration of \model{} at \textit{base} size., our next step is to scale it up. 
Pretraining LLMs at large scale introduces a new set of challenges.
Training large models is extremely slow and compute heavy which restricts the number of experiments that can be run with limited compute.
The size of LLMs also quickly reaches to a point where native training will require memory beyond limit of existing computing hardware, etc. 
As models gets deeper, optimization stability becomes a bigger issue with gradient exploding/vanishing, mixed precision over/underflow, etc. 
The model-generated training objective provides a good way to improve pretraining efficiency, but also requires proper calibration of the auxiliary and the main model to construct an effective learning curriculum.

In this section, we first discuss the configurations of \model{} at larger sizes, followed by the techniques we used to improve the computing efficiency for LLMs pretraining.
After that, we describe techniques we found critical to improve optimization stability of \model{} and discuss our findings during our scaling up attempts.



\subsection{Model Configuration}

How to configure a proper learning curriculum is a key research problem in curriculum learning~\citep{graves2017automated} and there is no exception in ELECTRA-style models.
On one hand the auxiliary model can not be too weak to produce hard enough training signals for the main Transformer. On the other hand a too strong auxiliary model will make the denoising task too hard and the main model will struggle. At the same time, the ``denoising difficulty" is hard to precisely measure and unlikely has linear correspondence with auxiliary model sizes. 
In this work, as the first attempt to scale up ELECTRA-style models, we keep the width of auxiliary models the same with the main. As the main model is scaled up, we run small ablations on the depth on auxiliary model for a limited amount of pretraining steps and pick the one that yield stable learning behaviors of the main Transformer. 

The configurations of \model{} at variant sizes are summarized in \ref{tab:model_configs}. \cx{here.} 
We follow the traditions at \textbf{base} and \textbf{large} in recent research~\citep{liu2019roberta, meng2021coco}. Different from previous practices~\citep{raffel2019t5, brown2020language}, at XL and XXL size, we emphasize on a balanced scale on network width and depth, instead of keeping the depth the same with smaller models and only blowing up the width.
Though it is a wide consensus that a deeper network often yield better generalization in deep learning, it is more challenging to increase the depth of LLMs as it yields more optimization stability problems, especially with Post-LayerNorm~\citep{xiong2020layer, shleifer2021normformer}. 
However, in this work, we aim to address the optimization stability issues using techniques described later in this section,  while keeping the benefits of Post Layernorm and deep networks in effectiveness.



\subsection{Techniques for Computing Efficiency}

We bring in two sets of techniques: ZeRO Optimizer and Customized Fused CUDA Operations, both yield remarkable efficiency benefits in parallel training for LLMs but impose minimum change to the model and implementation.

\textbf{ZeRO Optimizer.} With most common stochastic optimizers, the size of gradients and optimizer states grows linearly with model sizes. For example, with Adam, the optimizer state consumes even more GPU memory than the model itself, making it harder to fit larger models into single GPU memory. 
The DeepSpeed ZeRO optimizer~\citep{rajbhandari2020zero} provides various ways to partition the optimizer state, gradients, and model into each GPU in distributed training thus significantly reduces the GPU memory consumption of LLMs. 

Table \ref{tab:deepspeed_zero} shows the memory requirements when using variant stages of ZeRO. 
With ZeRO stage one we are able to fit a model with ~6B parameters without ZeRO in a 40GB A100 GPU. 
\input{Tabs/deepspeed_zero}.  
In stage one, ZeRO partitions optimizer states across GPUs. For example, with Adam, ZeRO stage 1 splits its 32-bit weights, as well as the first and second moment estimates) across multiple GPUs, thus significantly reduces the memory usage. This optimizer state sharding imposes no additional communication cost, by redesigning the communication loop between different GPUs during back propagation.
We choose ZeRO stage one in our scaling up experiments for its huge efficiency benefits but zero communication cost.


% We leverage ZeRO stage 1 where the optimizer states (e.g., for Adam optimizer, 32-bit weights, and the first, and second moment estimates) are partitioned across the processes, so that each process updates only its partition. Optimizer state sharding is sufficient to enable training a 6B model with no additional communication cost. Table \ref{tab:deepspeed_zero} shows that it would not be possible to fit a model with ~6B parameters without ZeRO in a 40GB A100 GPU. \\
% \input{Tabs/deepspeed_zero}

\textbf{Fused CUDA Operations.} Mixed-prediction, where training computations are performed in fp16 precision with only the main copy of model uses fp32 precision, is the standard for large scale training to reduce memory and communication cost.
However, it is often necessary to use fp32 for some operations to stick with fp32 for numerical stability, such as \textit{softmax} in the Transformer attention mechanism. 
In existing mixed-prediction implementations, e.g., with PyTorch's \textit{amp} package, the procedure is to first cast these tensors for these ops to fp32, perform the operation, and then cast the result back to fp16. This induces extra memory cost for casting and allocation.


This extra memory cost is, in fact, not necessary. We create custom CUDA kernels that fuse the fp32 casting and operations together at CUDA level, where we conduct do the casting and computing element-wisely, leveraging locality, without addition memories for access and allocation of intermediate results. In our experiments, fused ops provide a ~1.35x speed-up in base model pre-training. \cx{I like this but think we need more details here? There is a comparison from Guolin on the difference between FusedOps from previous infra and his implementation, and the relative speed up measurement. let's include that table and different levels of fusion here too? I like having the Algorithm boxes to describe FusedOps but I can't understand what they are and why they make a difference....}

\begin{algorithm}
\caption{Without Fused Ops}
\begin{algorithmic}[1]
\Procedure{stable\_op\_in\_fp32}{$x, F$} 
    \For {$i\ =\ 1\ to\ n$}     \Comment{Convert x to float}
    
        $t1[i] = x[i].float()$
    \EndFor
    \For {$i\ =\ 1\ to\ n$}     \Comment{Perform op}
        
        $t2[i] = F(t1[i])$
    \EndFor    
     \For {$i\ =\ 1\ to\ n$}    \Comment{Convert result to half}
     
        $y[i] = t2[i].half()$
    \EndFor \label{no_fused_ops}
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{With Fused Ops}
\begin{algorithmic}[1]
\Procedure{stable\_op\_in\_fp32}{$x, F$} 
    \For {$i\ =\ 1\ to\ n$}     \Comment{Element wise ops}
    
        $t1 = x[i].float()$
        
        $t2 = F(t1)$
        
        $y[i] = t2.half()$
        
    \EndFor  \label{with_fused_ops}
\EndProcedure

\end{algorithmic}
\end{algorithm}


\subsection{Techniques for Optimization Stability}


The difficulty of training transformers increases with depth. This instability also severely restricts the learning rate that can be used in pre-training which has a direct impact on model quality. We use Post-LayerNorm architecture which several previous works have shown to be harder to scale compared to Pre-LayerNorm but we have demonstrated in the ablation earlier that it can affect performance severely. \cite{liu2020understanding}, \cite{xiong2020layer}, and \cite{shleifer2021normformer} show there exists a gradient disparity in Post-LayerNorm architecture where expected gradients of the parameters near the output layer are larger than input layer resulting in unbalanced gradients which is the root cause of instability. \cx{split to a new paragraph here?}
We try several techniques to stabilize training and maintain curriculum as the model is scaled up. As the discrepancy in the number of layers in auxiliary and main model, we first try reducing peak learning rate in pre-training to slow-down the training for auxiliary model allowing main model to catch up. We also try reducing gradient norm to enable main model to catch up with the auxiliary model. \cx{So here we need to make a transition. before it is general techniques used in pretraining, later it is a relatively new one and we have more details.} To avoid large gradients in layers near the output layer, we adapt the dynamic initialization technique where the initial weights of FFNs are scaled by depth as follows. Given the transformer equations:

\begin{align}
MultiHead(Q, K, V) = Concat(h_1, ..., h_h)W^O \\
\quad
where\ h_i = Attention(QW^{Q}_{i}, KW^K_i, VW^V_i) \\
\quad
FFN(x) = max(0, xW_1 + b_1)W_2 + b_2 \label{eq:transformer}
\end{align}

We modify the following weights at initialization:
 
\begin{align}
W^O = W^O / \sqrt{layer_{id} + 1}\\
\quad
W_2 = W_2 / \sqrt{layer_{id} + 1} \label{eq:dynamic_init}
\end{align}

This reduces the weights at deeper layers thus reducing the variance and providing training stability. 

\subsection{Observations and Discussion:} 

Figure \ref{fig:DynamicInit} shows the Replace accuracy of the main model with and without dynamic initialization. The replace accuracy of main model stays at 0 when model is scaled up, reducing the learning rate helps main model to catch up with auxiliary model by delaying the latter's learning process as shown by slower reduction in replace rate, but the main model still struggles to keep up. Reducing the clip norm to 1 helps establish better curriculum and enable full pre-training but when dynamic initialization is enabled, the replace accuracy of the main model is much better at the same replace rate of auxiliary model thus demonstrating that it enables much training deeper model with more stability and better performance. Therefore, we enable dynamic initialization is METRO-XL and XXL pre-training.

\input{Figs/DynamicInit}

\input{Figs/XXL}

As the generator is shallower than discriminator, the effect of discrepancy increases while scaling up. \ref{fig:XXL} shows an example of hyper-parameter tuning for METRO-XXL model. The auxiliary model is easier to stabilize as it is 8 layers deep whereas the main model is much deeper and tends to diverge while training unless the LR is reduced.


\input{Tabs/model_scale_results}
\cx{discuss our view of best strategy in scaling up stably here, also serving as a call for action? Here is may be where we discuss our new work that could be intergrated, including AMOS, MuP, and Xiaodong's dynamic Learning rate paper in ICLR?}







==> arxiv/task_form.tex <==
\subsection{Task Formulation in Fine-Tuning}
\label{subsec:task}
% Notes by xiaodong
% BEST results of MNLI is ft-ed with PDR + ANLI+SNLI with filtered by sequence length. 
% MNLI, Record, QQP, BoolQ are ft-ed from 5.4B model, while others from 1.5B.

For GLUE, we use the same task formulation as the official paper: MNLI, SST-2, MRPC, QQP, QNLI, RTE and WNLI as classificationt tasks and STS-B as a regression task. MNLI is directly fine-tuned from pre-trained {\model} via PDR \cite{cheng2020pdr} and multi-task data augmentation \cite{liu2019mt-dnn} denoted as \textbf{MNLI+} while SST-2, MRPC, QQP, QNLI and RTE tasks are fine-tuned with PDR starting from the \textbf{MNLI+}  model. 

In cases of SuperGLUE, we also mainly follow the same setup as \cite{wang2019superglue} with a few modifications \footnote{Our code and script will be released at https://github.com/namisan/mt-dnn/tree/master/experiments/superglue.}: 
\begin{enumerate}
    \item \textbf{BoolQ}, \textbf{CB} and \textbf{MultiRC}: we follow the same input format as \cite{wang2019superglue, liu2019roberta} and fine-tune starting from the \textbf{MNLI+} model. 
    \item \textbf{COPA}: following \cite{liu2019roberta}, we concatenate the premise and each alternative with \textit{because} and \textit{so} markers instead of \textit{cause} and \textit{effect} question, respectively. 
    \item \textbf{ReCoRD}: we formulate it as a pairwise ranking task with one negative and positive entity for each (passage, query) pair as \cite{liu2019roberta}. At evaluation time, we pick the entity with the highest score for each question. Empirically, it obtains around 2 points of the F1 score improvement comparing with the span extraction as SQuAD \cite{rajpurkar2016squad}. 
    \item \textbf{WiC}: we just concatenate the marked word and the pair of sentence as input and only use the representation of [CLS] token for classification.
    \item \textbf{RTE and WSC}: we reused the our submission to the GLUE leaderboard. 
\end{enumerate}

